A Sticker is Worth a Thousand Words: Characterizing the Use of Stickers in WhatsApp Political Groups in Brazil

With the increasing use of smartphones, instant messaging platforms turned into important communication tools. According to WhatsApp, more than 100 billion messages are sent each day on the app. Communication on these platforms has allowed individuals to express themselves in other types of media, rather than simple text, including audio, videos, images, and stickers. Particularly, stickers are a new multimedia format that emerged with messaging apps, promoting new forms of interactions among users, especially in the Brazilian context, transcending their role as a mere form of humor to become a key element in political strategy. In this regard, we investigate how stickers are being used, unveiling unique characteristics that these media bring to WhatsApp chats and the political use of this new media format. To achieve that, we collected a large sample of messages from WhatsApp public political discussion groups in Brazil and analyzed the sticker messages shared in this context

==> Sections/clustering.tex <==



\subsection{Clustering stickers by visual similarity}


By clustering stickers using its perceptual hash we reach some patterns in sticker content.
Among the clusters, we found many variations of the same image. That means that users very often edit and fabricate their own versions of popular stickers. This is a common practice on WhatsApp and there are even groups dedicated exclusively to exchanging stickers between users~\cite{daniel22whatsappwebmedia}. In the context of the public politic groups collected in this work, many of them are related to main politicians in Brazil. 

Some clusters demonstrate an important characteristic of stickers: their use as a meme. These clusters put together analogous images that have a unique template but just differentiating by the text around them to instantiate a joke or a funny situation. This pattern is also followed by memes in which popular images (usually of a funny nature) are widely spread over the Internet with different variations and situations that fit into that meme category.


It is interesting to observe within some clusters, though, that very visually similar stickers may represent totally opposite ideas. Figure~\ref{fig:opposition} shows an example of a cluster that grouped two stickers very analogous, but shared in such a way that each sticker portrait opposes left- and right-wing candidates as they were prisoners, suggesting that some stickers are coopted by different groups and used in a contrary manner but using the same aesthetics.

\begin{figure}[h]
  \centering
  \subfigure[]{\includegraphics[trim={0 0 0 0},clip,width=0.35\linewidth]{stickers/lula_preso.png}}
  %\hfill
  \subfigure[]{\includegraphics[trim={0 0 0 0},clip,width=0.35\linewidth]{stickers/bolsonaro_preso.png}}
  
  \caption{Examples of stickers used by both political alignments}
  \label{fig:opposition}
\end{figure}






\subsection{Sticker Network}



\begin{figure}[h]
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=1.00\linewidth]{Figures/StickerNetwork_100.png}
  \caption{Visualization of network composed of top shared stickers. Nodes are stickers edges represent both appeared within same group.}
  \label{fig:nsfw_stickers}
\end{figure}


Average Degree: 811,397
Density: 0.778


Average Clustering Coefficient: 0,911
The Average Clustering Coefficient is the mean value of individual coefficients.


Eigenvector Centrality
Number of iterations: 100
Sum change: 0.005131657786253955



Diameter: 3
Radius: 2
Average Path length: 1.222775077785492

==> Sections/draft.tex <==


``A picture is worth a thousand words'' is a popular expression meaning that complex and sometimes multiple ideas can be transmitted by a single still image, which may conveys its essence more effectively than a verbal description.
Similarly, stickers are a form of visual media, popular in online messaging services, through which users can express emotion, nonverbal language, and state complex ideas. 

While online communication occupies a growing space in our daily lives, users increasingly demand new and more effective ways to express themselves through computers and smartphones.
Especially, during the COVID-19 pandemic, when this distance communication has become essential to keep in touch with family and friends, it also comes a need to show our emotions and feelings to people who are far from us.
In this scenario, sometimes just text-based communication may be not enough to demonstrate everything we want to tell. 
Even with emojis characters in text, this may prevent users from fully understanding the contextual subtlety and accuracy of the conversation. Users, however, may overcome such limitations with the usage of stickers~\cite{smileyface_stickers}, translating some form of language, interactions, gestures and symbols with this emerging multimedia messaging format.
%
WhatsApp itself, when introduced stickers within the app in 2018, refers them as ``stickers help you share your feelings in a way that you can't always express with words\footnote{\url{https://blog.whatsapp.com/introducing-stickers}}''.



Stickers are usually described as emoticons in the form of colored images~\cite{chen21multimedialanguage} as both can be used as visual reaction message or determine the feeling of the interlocutor during conversation but differ from in-line emoticons and emojis in diversity, complexity and usage~\cite{smileyface_stickers}. Also, they differ from simple static images as they can be animated as a GIF.
Sticker also is very related to memes~\cite{wang2019culturally}, often presenting a combination of picture and statement, typically with sarcastic or humorous intention~\cite{davison2012language}.
Both memes and stickers can be created based on personal experiences but also acquire inspirations from popular cultural products such as television shows and video games~\cite{ge2020memeticstickers}. 
Users publish meme images on Web and promote others to share through the imitation, alteration or transformation of the original~\cite{mememagic2021cscw}.


Instant messaging applications such as Facebook Messenger, Skype, WeChat, Line, and KaKao, Telegram, and WhatsApp have integrated stickers as a feature within their messages to complement the text messages. The popularization of this multimedia format have significant implications for how users engage in messaging as well as how they use those applications. With stickers, users express their identities, serving as a kind of social symbol that connotes social context and emotion for the messages~\cite{socialcontext07emoticons,derks08emoticons}.  



While WhatsApp's end-to-end encryption is great for user security, it also makes it quite difficult to measure the real impact of using stickers within the app. But there are other hints that capture the size of the success of this new form of media:
apps for creating stickers for WhatsApp, such as Sticker Studio and Sticker.ly, had more than 10M and 100M downloads, respectively, only for Android smartphones, and groups dedicated exclusively to exchanging stickers between users are among the most popular topics of public WhatsApp groups shared on the Web~\cite{daniel22whatsappwebmedia}. 
%
\footnote{\url{https://play.google.com/store/apps/details?id=stickermaker.android.stickermaker}}
\footnote{\url{https://play.google.com/store/apps/details?id=com.snowcorp.stickerly.android}}


Although stickers are very popular on WhatsApp, we lack of systematic analysis of use of stickers on a large scale within the messaging platforms ecosystem due the closed architecture of those systems. 

Users use sticker as same they use images on WhatsApp?
What are the characteristics of the sitckers sent on WhatsApp?
People can use stickers for abuse in chats on WhatsApp?


Stickers are a new form of media communication
Stickers are very popular on WhatsApp 
There is no systematic analysis of stickers on a large scale.




Memes are used not only for entertainment, but also expressions of deeper meanings such as political opinions~\cite{political_meme}.

https://www.whatsonweibo.com/the-power-of-chinas-internet-memes/






%\cite{smileyface_stickers} As mobile instant messaging has become a major means of communication with the widespread use of smartphones, emoticons, symbols that are meant to indicate particular emotions in instant messages, have also developed into various forms. The primary purpose of this study is to classify the usage patterns of emoticons focusing on a particular variant known as "stickers" to observe individual and social characteristics of emoticon use and reinterpret the meaning of emoticons in instant messages. A qualitative approach with an in-depth semi-structured interview was used to uncover the motive in using emoticon stickers. The study suggests that besides using emoticon stickers for expressing emotions, users may have other motives: strategic and functional purposes



